DynamoNet: Dynamic Action and Motion Network

In this paper, we are interested in self-supervised learning the motion cues in videos using dynamic motion filters for a better motion representation to finally boost human action recognition in particular. Thus far, the vision community has focused on spatio-temporal approaches using standard filters, rather we here propose dynamic filters that adaptively learn the video-specific internal motion representation by predicting the short-term future frames. We name this new motion representation, as dynamic motion representation (DMR) and is embedded inside of 3D convolutional network as a new layer, which captures the visual appearance and motion dynamics throughout entire video clip via end-to-end network learning. Simultaneously, we utilize these motion representation to enrich video classification. We have designed the frame prediction task as an auxiliary task to empower the classification problem. With these overall objectives, to this end, we introduce a novel unified spatio-temporal 3D-CNN architecture (DynamoNet) that jointly optimizes the video classification and learning motion representation by predicting future frames as a multi-task learning problem. We conduct experiments on challenging human action datasets: Kinetics 400, UCF101, HMDB51. The experiments using the proposed DynamoNet show promising results on all the datasets.

==> old_stuff.tex <==
\iffalse
\begin{enumerate}
\item Similar strategy as dynamic image enhancement.
\item What is action recognition? How can we encapsulate the dynamic motion? Would it be able to help if we can  learn-to-recognize only the dynamic (i.e. motion) fine-grained segments that to in a video level?
%\item Given that the dynamism is learned, a straight forward effectiveness can be shown for action ancticipation.
\item Incorporating visual learning and motion representation in one model, in comparison to model that use two-stream like architecture.
\item Multi task learning: classification and frame prediction.
\end{enumerate}

\section{Example text action.}
Humans are often good at imagining how a scene will change over time even from just a single snapshot. For instance look at these images based on the position of the girl many would guess that she is moving her leg as she exercises however can you tell if her leg is moving up or down? This is much harder question to answer, there is often an intrinsic ambiguity to the direction of the motion. In this work, we propose a probabilistic content-aware motion prediction model that learns the conditional distribution of future frames and allows us to sample and visualize the many possible ways that an input image is likely to change. Our algorithm is based on the VAE, the network takes the current frame and a random variable $Z$ sampled from a Gaussian distribution as input and outputs a future frame by taking different samples $Z$ as input the network can generate different future frames. The network structure is based on a novel cross convolutional layer. Given an input frame the network first decomposes the image into several layers then each layer is convolved with an image dependent motion kernel through a cross convolutional layer. These motion kernels are decoded from the random variable $Z$, this process generates the motion for each image layer. Finally all the layer are combined together to generate a next frame image. At training time, we add a motion encoder to learn the random variable $Z$ from two consecutive input frames, we can then train the network end-to-end. We present motion prediction results on three different datasets.
Here we show a sample of training data from a simple X dataset, and random synthesis results for the specified input image. Notice that although the same input image was used in generating each of these results, each results motion is slightly different. Testing images were not selected from the same videos, as we used to generate training images. We also run a study to evaluate our motion prediction synthesis results.

Successful predicting the future will demonstrate the computers understanding of object in the scene. One straight forward apporach would be discriminative training to predict the next 3 second frame, but our world is full of uncertainty. Its not the predictions are wrong, its just an intrinsic ambiguity in the prediction. There are multiple motions associated with  the inputs snapshot, and the discriminative method cannot model this uncertainty. So in order to model the uncertainty of the future frame, we can instead use probabilistic formulation. Unrealistic stretching is not ok, although maybe if we are lucky a few motion fields are going to be consistent with the input image. It is unlikely to happen if we ignore the image content during the sampling. There are only a few motion fields that are consistent to the input image.

There is a strong correction between images and their respective motion fields, we would also like to model this connection to avoid the unrealistic  motion such as unrealistic stretching girl.

In this work, we want to predict the future, and correlation between the image and the motion.
Given an input image, we want to predict the future, they all are consistent with the input. Let us consider, how we generate one future frame, many frameworks propose to synthesize image from scratch, but our synthesis based on segments which we believe can model better image-content and motion. \textbf{To do so, we crop the image to different segments, we then transform each segment, thus keeping the torso unchanged and rotate the leg, atlast we combine all the segments to generate the future frame. Now to generate different future frame,  we can keep the segmentation part unchanged, and transform the segments differently, e.g. we rotate the leg, and the different future frame is generated. }

In that case, we can generate natural future frame. Shortcoming: blur, when motion is small, awesome results, when the motion is large, it may introduce artifacts. We believe that large motion can't be modeled by simple convolution of each segment. We might need a more complicated segment to solve this problem.  Although our method generates artifacts, it often generates realistic looking results.

Contributions: (1) Sample multiple future frames that are consistent with the input. (ii) Synthesizing frames by transforming segments. (iii) Learn a motion representation without supervision.

\fi



\section{Proposed Method}
The proposed end-to-end network is designed to simultaneously classify action and learn motion representation by predicting the short-term future frames. The main section of the network is a 3D convolutional network \cite{3dresnet,oureccv} and has two branches to do classification and dynamic frames prediction. The input to the network is a sequence of the frames with 16 or 32 stack of frames in different experimental setup which is called video clip in this paper.

Actually the frame prediction part of network extracts the internal motions and variations in the video clip by generating dynamic filters to predict next frame given the previous one. So if the input clip consists the ${t:t+n}$ frames the network reconstructs and predicts ${t+1:t+n+1}$ which ${n=16,32}$. By extracting this intra-information from the clip, we have some sort of motion representation from the same clip since the generated filters are demonstrating the variation info of frames. This representation can accompany the classification representation branch to have more solid action classifier as well. So basically, we want to reconstruct the same clip without first frame plus next frame right after the clip. In the next, we elaborate the method details.

\subsection{Dynamic Motion Filters}

\begin{figure}[t]
\centering
{\includegraphics[width=1\columnwidth]{fig2.pdf} } 
\caption{dynamic filter function}\vspace{-0.5cm} 
\label{fig:dynfilter}
\end{figure}

Given a video clip $x \in \mathbb{R}^{H\times W \times t}$, the network produces dynamic filters to create $\^x \in \mathbb{R}^{H\times W \times (t+1)}$ where $t$ is clip duration and $W,H$ are clip frames width and height. So as before mentioned, the predictor part of network is defined as:

\begin{equation}
\^x_{t+1} = G(x_{t} \circledast F_{t}).
% z_{tcb}=\dfrac{1}{W \times H \times T} \sum_{i}^{W}\sum_{j}^{H}\sum_{t}^{T}{x_{ijt}} \ .
\end{equation}

\begin{figure*}[t]
 \centering
 \includegraphics[width=2\columnwidth]{fig3.pdf}
 \caption{\textbf{DynamoNet}} 
  \label{fig:DAMnet}
 \end{figure*}

where $G$ is the part of network function to produce the frames by generated filters $F$. As shown in Figure~\ref{fig:dynfilter}, the network yields 16 or 32 (depending on the size of input clip) motion filters to be convolved with the input clip to have the generated clip as output. In our experiments we have tested filter with different sizes like $4\times4$ or $5\times5$ and filters with size of $5$ performs the best.

Inspired by dynamic filter network \cite{bertDyn}, we believe that to exploit a nice representation of motions in video clips, dynamically generated filters is a robust solution to capture variations. These filters are variant and dependant on the input clip and for each batch of frames different filters will be generated. That is why they are called dynamic.
If input clips has a length of 16, the network generates 16 filters and each of these filters will be convolved with corresponding input frames to synthesize the next frames. So the main difference in our method for generating next frames in compassion to other method is that we do not generate frames directly by convolution and de-convolution layers but we use these layers to obtain some motion filters to reconstruct the next frames. Our network configuration and the learning scheme helps to learn the pixel motion information in an spatio-temporal regime.



As mentioned before, our network has two tasks: Recognition and Frames prediction which we need to objective function. For the frame prediction part, the Huber loss function which is used comes as:\\
\begin{equation}
% \^x_{t+1} = G(x_{t} \circledast F_{t}).
\mathcal{L}_{FP} =\left\{
                \begin{array}{ll}
                  \frac{1}{2}||\^x_{t+1}-x_{t+1}||^{2}_{2}\quad \textbf{if} \quad
                  ||\^x_{t+1}-x_{t+1}||_{1} < \delta \\
                  \\
                  \delta||\^x_{t+1}-x_{t+1}||_{1} - \frac{1}{2}\delta^{2}\quad otherwise
                \end{array}
              \right.
\end{equation}

FP stands for frame prediction and the $\delta$ threshold is set to $0.01$. More details about the training and the network will come in the experiments section.


 

\subsection{Action Recognition}
Our main idea to pick a network with a high capacity to do classification and frame prediction was a 3D CNN. So we use 3D-STCNet\cite{stcnet} or 3D-ResNet\cite{3dresnet} as the main part of the network. These CNNs showed promising performance for action classification both in accuracy and speed in different datasets. The 3D convolutional layers handle the appearance and temporal information in a better shape than 2D networks. So 3D-STCnet/ResNet are good candidates to extract information for action classification and motion analysis.

The both of network branches are trained together, therefore we have the action representation and motion filters at the same time. So, we flatten the motion filters and concatenate them together to become as a single vector and we call it dynamic motion representation (DMR). The action representation and DMR will be concatenated together and pass to the classification cost function. With this way we incorporate the motion information to classification task also.

\textbf{Learning the Network:} During the training, we minimize sum of the two losses for frame prediction and action classification.
So the total loss is:
\begin{equation}
% \^x_{t+1} = G(x_{t} \circledast F_{t}).
\mathcal{L}_{H} =\alpha\mathcal{L}_{FramePrediction} + \beta\mathcal{L}_{Classification}
\end{equation}

where $\alpha,\beta$ are losses weights and both of the tasks are optimized together. It can be noted that the trained DMR is optimized to picture the best motion information for specific actions in this training setup.

\subsection{Unsupervised Training}
If we remove the classification branch and just keep the dynamic filter and frame prediction part, an unsupervised video learning pipeline can be obtained. The most important aspect of videos are meaningful motions. So one of the most practical way to train a video understanding network in an unsupervised way is trying to re-create the future frames and also extract the motion information. The is a self supervision signal in the sequences of frames.

We have experimented the method with number of unlabeled videos and trained the network from scratch. It proves that such a unsupervised pre-training network can be very impactful and decreases the need for more videos to train 3D CNN for action classification from scratch.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this paper, we propose to extend the training of ConvNets-based action classification to incorporate the high-level goal to learn \textit{action-specific} motion representation via future frame prediction. Our contribution is a method that jointly optimizes a ConvNet for video action classification and future frame prediction as a multi-task learning problem. We achieve this by adaptively learning the motion features on a \textit{video-specific} basis via dynamic motion filters, which enables the motion prediction model to selectively utilize only those motion features that lead to improved video classification. 

% The main contribution of our work is to discover and learn video-specific internal motion representations for improved video classification. We achieve this by adaptively extracting informative features by predicting the short-term future frames to improve classification.
% We believe predicting (or reconstructing) the future frames selectively transfers the \textit{fundamental notion} of motion content to the filters, which in turn improve the overall effectiveness of the motion representations. The motion representation learning is jointly optimized along with the video classification as a multi-task learning problem. Using short-term future frame prediction as a proxy task is promising, and we clearly show that this works for an accurate action recognition in videos.

Since we understand the vital role of motion feature representation, we propose to use the dynamic convolutional filters to dynamically learn the \textit{video-specific} motion features with an video classification objective (see Fig.\ref{fig:front} for a graphical overview). Our paper is inspired from~\cite{dfn,dyncnn}. However, while Brabandere et al.~\cite{dfn}  applies the dynamic filters to transform an angle to a filter (steerable filter) and Sharma et al.~\cite{dyncnn}  emulates a range of enhancement filters to generate image enhancement methods. We used the same terminology as in~\cite{dfn,dyncnn}. In contrast to these works, our work differs substantially in technical approach and the application scope. Our model is designed to learn  motion representation by predicting the short-term future frames and  simultaneously classifying actions. Our network takes the current video-clip with $T$ frames and generates $T+1$ future frames using  $T$ dynamic motion kernels or dynamic filters. The network structure is based on 3D ConvNets. Specifically, given an input video-clip $x$ with $T$ frames the network generates $T$ dynamic motion kernels ($F_{T}$) to predict the consecutive next frame given the previous one i.e. $F_{t}: x_{t} \rightarrow \^x_{t+1}$, $t \in \{1,\ldots,T\}$. These filters are video dependent motion kernels and are conditioned on the input and therefore vary from one sample to another during training and testing phase, which means that the filter dynamically extracts important motion representation from a given input. Further, we utilize these $T$ $d$-dimensional dynamic motion features along with STC-ResNext~\cite{stcnn,resnet3d} 3DConvNet features for video classification. Moreover, we believe the dynamic motion kernels capture the important concepts of motion representation from the temporal cue and the extracted motion features are robust and compact global temporal representation for the whole video, this makes them a perfect fit for action recognition task well. Note that, the goal of this paper is not only to achieve high performance, but also to show that a better motion representation can be obtained from an ample number of consecutive frames, similar inspiration could be taken from handcrafted IDT~\cite{idt}. Our method is evaluated on three challenging benchmark action recognition datasets, namely UCF101, HMDB51 and Kinetics 400. We experimentally show that the 3D ConvNets when combined with our dynamic motion filters (Sec.~\ref{sec:exp}) achieve state-of-the-art performance on UCF101 (97.8\%), HMDB51 (76.8\%) and Kinetics 400 (70.4\%).

